Cleaning Denial Constraint Violations through Relaxation

Data cleaning is a time-consuming process that depends on the data analysis that users perform. Existing solutions treat data cleaning as a separate offline process that takes place before analysis begins. Applying data cleaning before analysis assumes a priori knowledge of the inconsistencies and the query workload, thereby requiring effort on understanding and cleaning the data that is unnecessary for the analysis. We propose an approach that performs probabilistic repair of denial constraint violations on-demand, driven by the exploratory analysis that users perform. We introduce Daisy, a system that seamlessly integrates data cleaning into the analysis by relaxing query results. Daisy executes analytical query-workloads over dirty data by weaving cleaning operators into the query plan. Our evaluation shows that Daisy adapts to the workload and outperforms traditional offline cleaning on both synthetic and real-world workloads.

==> logical_optimizations.tex <==
\vspace{-1.5em}
\section{Cleaning-aware \\ Query Optimization \& Planning}
\label{sec:loglevel_optimizations}

In this section, we present how we inject cleaning operators at the logical level, and show optimizations that enable 
an optimal placement of cleaning operators in the query plan.
We support queries, with Select, Join and Group by clauses.  %\TODO{add query template}
The template of the supported queries can be found in the technical report.
%The template of the supported queries is the following:
%\vspace{-0.5em}
%\begin{minted}[escapeinside=||,fontsize=\footnotesize]{sql}
%SELECT <SELECTLIST>
%FROM <table name> [,(<table name>)]
%[WHERE <col><op><val> [(AND/OR <col><op><val>)]]
%[GROUP BY CLAUSE]
%\end{minted}
%\vspace{-0.5em}
%CONDITIONS=<col><op><val> or col> [(AND/OR <col><op><val>)]
%%%%%%%%%%%%%%%%%%%%%%%%ADD%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\noindent [] and () indicate optional and repeated elements. $op$ takes values $=,\neq, <, \leq, >, \geq$.
%In the case of joins, we assume equi-joins.
We focus on flat queries to stress the overhead of the cleaning operators over the corresponding query operators.
%We introduce two types of cleaning operators depending on the underlying query operators in the logical plan.
%We use the operator $clean_\sigma$ for the case of select queries, and the operator
%$clean_\Join$ for join queries . The two operators differ in that  $clean_\sigma$ gets
%as input a single relation, whereas  $clean_\Join$ gets two relations.
%The operator $clean_\sigma$ gets as input the output of a \textit{select} operator and cleans the
%part of the dataset that qualifies the select condition using extra tuples from the dataset. Then, it outputs
%the enlarged set of qualifying tuples, and updates the dataset with the modified tuples.
%The implementation of  $clean_\sigma$ is presented in Section \ref{sec:query_relax}.
%The $clean_\Join$ operator gets as input the output of a join operator, and then extracts
%the qualifying parts from both tables. Afterwards, $clean_\Join$
%cleans the corresponding erroneous tuples separately in each relation, updates the join result
%and re-checks for violations. Thus, $clean_\Join$ might require multiple iterations until no
%changes are required in the join result. The implementation of  $clean_\Join$ is presented in Section \ref{sec:query_relax}.


%\begin{figure*}[t]
%	\begin{subfigure}{0.42\textwidth}
%			\centering
%		\includegraphics[width=0.7\textwidth]{figures/plan2}
%		\vspace{0.005em}
%		\caption{Pruning extra violation detection when there is no filter condition prior to the join operator. }
%		\label{fig:no_filter_plan}
%	\end{subfigure}	
%	\hspace{4em}
%	\begin{subfigure}{0.42\textwidth}
%			\centering
%		\includegraphics[width=0.8\textwidth]{figures/plan1}
%		\caption{Pruning extra error detection when there is a filter on the attributes that do not participate in a rule.}
%		\label{fig:rhs_plan}
%	\end{subfigure}
%	\vspace{-0.5em}
%	\caption{Logical level optimizations.}
%	\label{fig:optimized_plan}
%	\vspace{-1em}
%\end{figure*}

\subsection{Cleaning operators in the query plan}
\label{subsec:cleaning_ops}

The logical planner detects the query operator attributes that appear in a rule, and injects the appropriate
cleaning operators in the query plan. 
The planner pushes cleaning operators down, closer to the data, to avoid propagating errors in the plan. 
Deferring the execution of a cleaning task requires a) redundant cleaning
to detect errors that have propagated from the underlying query operators, and/or
b) recomputing the underlying query operators that are affected by the errors.
For example, consider relations $R$ and $S$, and a query with a select condition over an attribute $R.a$ of $R$ that participates in a rule, 
followed by a join $R.a \bowtie S.a$ where $S.a$ also participates in a rule of $S$. Executing the cleaning task after the
join, might result in altering the qualifying part of $R$ by adding an extra probabilistic tuple. If the extra tuple
matches with an unseen tuple of $S$, then it will update the join result. Subsequently, the operator needs to re-check for errors over the extra accessed tuples of $S$,
which induces a redundant overhead for query execution.
Thus, placing cleaning operators early in the plan avoids extra effort to fix propagated errors.

%%%%%%%%%%%%%%%%%%%%%%%%%%%ADD%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fig. \ref{fig:no_filter_plan} shows an example query plan with a $clean_{\bowtie}$ operator.
%Given two rules involving the zip code of $R$ and $S$, the planner detects the overlap
%of the join operator with the rules, and injects the $clean_{\bowtie}$ operator.
%To avoid recomputing the join, $clean_{\bowtie}$ sends only
%the new tuples of each relation to the join operator. Thus, the second join corresponds to an incremental
%join, which updates the already computed result. The final result consists of the union of the join outputs.

%shows an example query plan which involves cleaning
%operators. Specifically, assume two relations $R$ and $S$, which both involve FD violations. 
%After the join operation, the plan adds a cleaning 
%operator $clean_\Join$ which separately cleans each relation and then updates the join result
%with the additional tuples that result from the cleaning task.

%\subsection{Plan Simplification}
%To prune unnecessary checks, the optimizer examines the query and detects how the
%violations affect the correctness of the query result.
%In the following, we distinguish among different cases in which the query operators and the rules interfere, 
%and describe the candidate optimizations that the system can apply in the query plan.
%
%\textbf{Join without select condition on individual tables}: In the case where there is no select condition 
%prior to the join operator, the \textit{query and clean} process requires a single iteration. 
%Consider a join between relations $R$ and $S$ which both involve violations on the join attribute.
%In this case, the cleaning operator might add new tuples to both relations. However, the extra tuples of 
%$R$ will match with tuples of $S$ which already 
%exist in the join result since they  have to belong to the intersection of the join keys of $R$ and $S$. 
%Thus, no extra violations will be detected
%since the added tuples have already been examined and cleaned. Similarly for the extra tuples of $S$.
%Figure \ref{fig:no_filter_plan} shows an example plan simplification in the case of a join over two relations
%that do not involve any prior select condition. The plan simplification transforms the iterative clean and join
%task into a single clean and join operation. To avoid recomputing the join, $clean_\Join$ sends only
%the new tuples of each relation to the join operator. Thus, the second join corresponds to an incremental
%join, which updates the already computed result. The final result consists of the union of the join outputs.
%
%\textbf{Join over a clean attribute with a filter condition over the erroneous attributes}: In the case where there 
%is a filter condition involving attributes that participate in a constraint, and there is no overlap with the join attribute, then the extra 
%tuples that will be added after cleaning the erroneous attribute, will not satisfy the select condition. Thus, a single iteration is required. 
%Figure \ref{fig:rhs_plan} shows a simplification of a plan involving a join over 
%a select condition on an erroneous attribute.
%For relation $R$ no extra cleaning is required. For $S$, the plan applies the
%data cleaning task, and then updates the join result, because the extra tuples of $S$ that the cleaning
%operator will produce might match with the qualifying tuples of relation $R$.

%\textcolor{red}{TODO: generalize for random queries}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ADD%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.23\textwidth]{figures/plan2}	
%	\caption{Before and after injecting $clean_{\bowtie}$ inside a plan with a join over a potentially erroneous attribute. }
%	\label{fig:no_filter_plan}
%	\vspace{-1.7em}
%\end{figure}

\input{cost_model}
